Decoding the Galactic Twirl: The Downfall of Milky Way-mass Galaxies Rotation Curves in the FIRE Simulations

Recent measurements of the Milky Way rotation curve found a sharp decline at around $15$-$20$ kpc from the center of the Galaxy, suggesting that the Galactic dark matter halo is much less massive than predicted by other dynamical tracers. To address this tension, we study the validity of the assumptions made in calculating the Milky Way's rotation curve. To do so, we apply Jeans' equation, the current standard approach of measuring rotation curves, to three cosmological zoom-in simulations of Milky Way-like galaxies from the FIRE-2 Latte suite. Using synthetic Gaia surveys, we replicate the sample selection process and calculation employed in measuring the Milky Way rotation curve. We examine four failure modes of this calculation and find that the measured curves deviate from the true curve by $5$-$20\%$ rather than below $5\%$, as estimated by previous works. Interestingly, there is a large galaxy-to-galaxy variance, and different systematics dominate different galaxies. We rederive the Milky Way's dark matter density profile with the rotation curve while incorporating systematics from the simulations. The posterior distribution of the density profiles is consistent with a fiducial NFW profile when assuming a gNFW profile for dark matter. We find that the virial mass, $7.32^{+1.98}_{-1.53}\times10^{11}~M_{\odot}$, consistent with other probes of the Milky Way's mass. However, we recommend that the field moves away from relying solely on the rotation curve when studying the dark matter profile, and adopts methods that incorporate additional probes and/or do not heavily depend on assumptions described in this study.

==> tab01.tex <==
\begin{deluxetable*}{cccc}
\caption{
Summary of curves derived in this study for each of the three galaxies, and the associated failure modes and assumptions.
\label{tab:curves}
}
\tablehead{
% \colhead{} & \colhead{\Ananke\ curves from Jeans equation} & \colhead{\Fire\ curves from Jeans equation} & \colhead{\Fire\ curves from \agama\ fitted potential} \\
\colhead{} & \colhead{\textbf{\Ananke\ curves}} & \colhead{\textbf{\Fire-2 curves}} & \colhead{\textbf{\Fire-2 curves}} \\
\colhead{} & \colhead{\textbf{from Jeans equation}} & \colhead{\textbf{from Jeans equation}} & \colhead{\textbf{from \agama\ fitted potential}}
}
\startdata
Selection function-biased tracer population & Affected & Unaffected & Unaffected \\
\hline
Higher order asymmetric drift correction & Affected & Affected & Unaffected \\
Inaccurate tracer profiles &  &  &  \\
\hline
Dynamical disequilibrium & Affected & Affected & Unaffected \\
\hline
Axis asymmetry  & Affected & Affected & Unaffected\tablenotemark{$\ast$} 
\enddata
\tablenotetext{\ast}{The fit is performed on all simulation particles but principally assumes axis symmetry. See texts for details.}
\end{deluxetable*}

==> tab02.tex <==
\begin{deluxetable*}{lrrrrrrrr}
\caption{
Summary of systematic uncertainties from the four failure modes in this study for each of the three galaxies.
\label{tab:sys_sum}
}
\tablehead{
% \colhead{} & \colhead{\Ananke\ curves from Jeans equation} & \colhead{\Fire\ curves from Jeans equation} & \colhead{\Fire\ curves from \agama\ fitted potential} \\
\colhead{} & \multicolumn{2}{c}{Biased population} & \multicolumn{2}{c}{Asym. drift correction} & \multicolumn{2}{c}{Axis asymmetry} & \multicolumn{2}{c}{Dynamical disequilibrium}\tablenotemark{$\ast$}  \\
\hline
\colhead{} & \colhead{Max. bias} & \colhead{Direction} & \colhead{Max. bias} & \colhead{Direction} & \colhead{Min. unc.} & \colhead{Max. unc.} & \colhead{Min. unc.} & \colhead{Max. unc.}
}
\startdata
m12i & $7\%$ & Positive\tablenotemark{$\dagger$} & $16\%$ & Negative & $1\%$ & $17\%$ & $0.4\%$ & $7\%$ \\
% \hline
m12f & $16\%$ & Positive & $7\%$ & Negative & $2\%$ & $7\%$ & $0.5\%$ & $2\%$ \\
% \hline
m12m & $6\%$ & Positive & $12\%$ & Negative & $0.4\%$ & $5\%$ & $0.3\%$ & $2\%$
\enddata
\tablenotetext{\ast}{Values reported here are estimated from the $z=0$ snapshots of the galaxies, where there are no recent major merger events. See Section~\ref{sec:res_dd} for a case of recent merger effects on m12f.}
\tablenotetext{\dagger}{The data point at the largest $R$ in Figure~\ref{fig:sys_sf_rel} for m12i has technically the greatest bias ($9\%$) in the negative direction. Since this is a single data point with a large statistical uncertainty and the rest of the data points all show positive bias, we opt to report the greatest bias in the positive direction here.}
\end{deluxetable*}

==> tab03.tex <==
\begin{deluxetable*}{lccc}
\caption{\textsc{emcee} fitted results for Einasto and gNFW dark matter halo profiles. We report the median of the posterior distribution and the 16$^{\rm{th}}$ to 84$^{\rm{th}}$ percentile as uncertainties. 
% A full analysis of systematic uncertainties will be presented in a future study.
NOTE: both profiles shown problematic behaviors in the posterior distribution and are thus only shown here for completeness as discussed in Section~\ref{sec:comp_mw}. 
The virial masses and radii are inconsistent at $2\,\sigma$ between the two best-fit profiles, suggesting the physical interpretation of the same data is sensitive to the chosen functional form of the underlying dark matter profile. 
}
\label{tab:fit_res}
\tablehead{
\colhead{} & 
\colhead{Einasto} & 
\colhead{gNFW} & 
\colhead{Prior} 
}
\startdata
\textbf{Normalization Mass ($M_0$)} & \MnorE & \Mnorg & $[0.1,1000]\times10^{11}$~\msun\tablenotemark{$\ast$} \\
\textbf{Scale Radius ($r_s$)} & \rscaE & \rscag & $[0,20]$~kpc \\
\textbf{Slope Parameter ($\alpha,\beta$)} & \slopE & \slopg & $[0,5]$ \\
\hline 
\textbf{Virial Mass ($M_{200}$)} & \MvirE & \Mvirg & -- \\
\textbf{Virial Radius ($r_{200}$)} & \rvirE & \rvirg & -- \\
\textbf{Concentration ($c_{200}$)} & \concE & \concg & -- \\
\textbf{Local Dark Matter Density ($\rho_{\rm{DM},\odot}$)} & \rhoSE & \rhoSg & -- \\
% \textbf{$J$-factor ($J(\theta < 15^{\circ})$)} & \JfacE & \Jfacg & -- \\ % Not doing this for now
\hline 
\textbf{$\chi^2$ per d.o.f. ($\chi_{\nu}^2$)} & \chisE & \chisg & --
\enddata
\tablenotetext{\ast}{Fitted in logarithmic scale.}
\end{deluxetable*}
